HomOpt: A Homotopy-Based Hyperparameter Optimization Method

Machine learning has achieved remarkable success over the past couple of decades, often attributed to a combination of algorithmic innovations and the availability of high-quality data available at scale. However, a third critical component is the fine-tuning of hyperparameters, which plays a pivotal role in achieving optimal model performance. Despite its significance, hyperparameter optimization (HPO) remains a challenging task for several reasons. Many HPO techniques rely on naive search methods or assume that the loss function is smooth and continuous, which may not always be the case. Traditional methods, like grid search and Bayesian optimization, often struggle to quickly adapt and efficiently search the loss landscape. Grid search is computationally expensive, while Bayesian optimization can be slow to prime. Since the search space for HPO is frequently high-dimensional and non-convex, it is often challenging to efficiently find a global minimum. Moreover, optimal hyperparameters can be sensitive to the specific dataset or task, further complicating the search process. To address these issues, we propose a new hyperparameter optimization method, HomOpt, using a data-driven approach based on a generalized additive model (GAM) surrogate combined with homotopy optimization. This strategy augments established optimization methodologies to boost the performance and effectiveness of any given method with faster convergence to the optimum on continuous, discrete, and categorical domain spaces. We compare the effectiveness of HomOpt applied to multiple optimization techniques (e.g., Random Search, TPE, Bayes, and SMAC) showing improved objective performance on many standardized machine learning benchmarks and challenging open-set recognition tasks.

==> algorithm.tex <==
\usepackage{algorithm}
\usepackage{algorithmic}

\begin{algorithm}[H]
    \caption{Homotopy Optimization Method for Hyperparameter Optimization (HOM)}
    \begin{algorithmic}[1]
        \Procedure{HOM}{$inner\_method, k, iterations, jitter\_strength, warm\_up, trial\_data, domains$}
        \State $params \gets$ hyperparameters to be used for next trial
        \State $eps \gets$ size of the interval of each hyperparameter domain being searched
        \State $n\_trials \gets$ number of completed trials so far
        \State $gam1 \gets$ GAM to fit on a subsampling of the most recent trials
        \State $gam2 \gets$ GAM to fit on all completed trials
        \If{the effective size of each hyperparameter domain has not been set yet}
            \State Compute it based on the bounds of each domain
        \EndIf
        \If{the number of completed trials is less than the warm up value or the number of completed trials modulo 5 is either 0 or 2}
            \State Generate parameters using the inner method
        \ElsIf{the number of completed trials modulo 5 is either 3 or 4}
            \State Sample random strategy hyperparameters and compute corresponding function evaluations around the observed minimum in the domain bounded by a distance threshold of M
        \Else
            \State Extract the hyperparameters and losses from the trial data and get the index of the best observed hyperparameters/loss pair
            \State Shift the data to have zero mean and unit variance
            \State Fit GAM1 to a subsampling of the most recent trials using $k$ as the fraction of completed trials
            \State Fit GAM2 to all completed trials
            \State Create a flattened array of inputs to minimize
            \State Set the threshold value to 1.0 and the step size to 1/iterations
            \For{each iteration from 1 to iterations}
                \State Minimize the function \Call{fun\_gam1}{$params$, $gam1$, $gam2$, $t$} with the current $X0$, $GAMs$, and threshold, and update $X0$ for the next round
            \EndFor
            \State Predict scores for the recorded $X$ values and determine the best
            \State Rescale the optimal parameters to the original domains
            \State $params \gets$ optimal hyperparameters obtained in step 2, 3, or 4
        \EndIf
        \State \textbf{return} $params$
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
    \caption{Function to be Minimized}
    \begin{algorithmic}[1]
        \Procedure{fun\_gam1}{$params$, $gam1$, $gam2$, $t$}
        \State $params \gets$ hyperparameters to be evaluated
        \State $y1 \gets$ predicted loss from GAM1
        \State $y2 \gets$ predicted loss from GAM2
        \State \textbf{return} $t * y1 + (1-t) * y2$
        \EndProcedure
    \end{algorithmic}
\end{algorithm}






==> tables/EVM.tex <==
\begin{table}
\centering
\caption{\textbf{Average percent improvement and standard error for the best observed loss over five trials of \HomOpt{} over the base methodology for each dataset and method for the open set benchmarks. Bold values indicate where \HomOpt{} outperforms the base methodology.}}
\label{tab:EVM}
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Dataset} & \multicolumn{4}{c}{Method}             \\
 & \textbf{bayes} &             \textbf{random} &              \textbf{smac} &                \textbf{tpe}                    \\
\midrule
LFW     &  \textbf{2.73} $\pm$ 0.35 &  \textbf{1.28} $\pm$ 0.21 &  \textbf{2.74} $\pm$ 0.31 &  \textbf{4.29} $\pm$ 0.86 \\
MNIST   &  \textbf{6.82} $\pm$ 0.11 &  \textbf{1.66} $\pm$ 0.14 &  \textbf{3.00} $\pm$ 0.30 &  \textbf{3.19} $\pm$ 0.14 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/EVM_all.tex <==
\begin{table}[ht!]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Method}} &
  \textbf{Validation F1} &
  \textbf{Validation Accuracy} &
  \textbf{Validation NMI} &
  \textbf{Testing F1} &
  \textbf{Testing Accuracy} &
  \textbf{Testing NMI} \\ \midrule
\multicolumn{1}{c}{\textbf{Random}} &
  \multicolumn{1}{c}{0.8982 $\pm$ 0.006} &
  \multicolumn{1}{c}{0.8958 $\pm$ 0.007} &
  \multicolumn{1}{c}{0.7547 $\pm$ 0.014} &
  \multicolumn{1}{c}{0.8988 $\pm$ 0.005} &
  \multicolumn{1}{c}{0.8969 $\pm$ 0.007} &
  \multicolumn{1}{c}{0.7579 $\pm$ 0.013} \\
\multicolumn{1}{c}{\textbf{PSHHO+Random}} &
  \multicolumn{1}{c}{\textbf{0.9160 $\pm$ 0.003}} &
  \multicolumn{1}{c}{\textbf{0.9127 $\pm$ 0.004}} &
  \multicolumn{1}{c}{\textbf{0.7889 $\pm$ 0.008}} &
  \multicolumn{1}{c}{\textbf{0.9039 $\pm$ 0.006}} &
  \multicolumn{1}{c}{\textbf{0.9022 $\pm$ 0.007}} &
  \multicolumn{1}{c}{\textbf{0.7657 $\pm$ 0.012}} \\
\multicolumn{1}{c}{\textbf{TPE}} &
  \multicolumn{1}{c}{0.8889 $\pm$ 0.011} &
  \multicolumn{1}{c}{0.8859 $\pm$ 0.011} &
  \multicolumn{1}{c}{0.7431 $\pm$ 0.022} &
  \multicolumn{1}{c}{0.8788 $\pm$ 0.004} &
  \multicolumn{1}{c}{0.8766 $\pm$ 0.004} &
  \multicolumn{1}{c}{0.7287 $\pm$ 0.009} \\
\multicolumn{1}{c}{\textbf{PSHHO+TPE}} &
  \multicolumn{1}{c}{0.9140 $\pm$ 0.003} &
  \multicolumn{1}{c}{0.9106 $\pm$ 0.004} &
  \multicolumn{1}{c}{0.7838 $\pm$ 0.005} &
  \multicolumn{1}{c}{0.8982 $\pm$ 0.007} &
  \multicolumn{1}{c}{0.8964 $\pm$ 0.006} &
  \multicolumn{1}{c}{0.7579 $\pm$ 0.012} \\
\multicolumn{1}{c}{\textbf{Bayes}} &
  \multicolumn{1}{c}{0.8771 $\pm$ 0.008} &
  \multicolumn{1}{c}{0.8749 $\pm$ 0.006} &
  \multicolumn{1}{c}{0.7200 $\pm$ 0.015} &
  \multicolumn{1}{c}{0.8669 $\pm$ 0.010} &
  \multicolumn{1}{c}{0.8655 $\pm$ 0.008} &
  \multicolumn{1}{c}{0.7054 $\pm$ 0.018} \\
\multicolumn{1}{c}{\textbf{PSHHO+Bayes}} &
  \multicolumn{1}{c}{0.9132 $\pm$ 0.002} &
  \multicolumn{1}{c}{0.9092 $\pm$ 0.003} &
  \multicolumn{1}{c}{0.7793 $\pm$ 0.003} &
  \multicolumn{1}{c}{0.8995 $\pm$ 0.003} &
  \multicolumn{1}{c}{0.8981 $\pm$ 0.004} &
  \multicolumn{1}{c}{0.7583 $\pm$ 0.004} \\
\multicolumn{1}{c}{\textbf{SMAC}} &
  \multicolumn{1}{c}{0.9034 $\pm$ 0.005} &
  \multicolumn{1}{c}{0.9001 $\pm$ 0.006} &
  \multicolumn{1}{c}{0.7650 $\pm$ 0.013} &
  \multicolumn{1}{c}{0.8924 $\pm$ 0.006} &
  \multicolumn{1}{c}{0.8907 $\pm$ 0.007} &
  \multicolumn{1}{c}{0.7468 $\pm$ 0.013} \\
\multicolumn{1}{c}{\textbf{PSHHO+SMAC}} &
  \multicolumn{1}{c}{0.9110 $\pm$ 0.006} &
  \multicolumn{1}{c}{0.9081 $\pm$ 0.005} &
  \multicolumn{1}{c}{0.7797 $\pm$ 0.009} &
  \multicolumn{1}{c}{0.8992 $\pm$ 0.004} &
  \multicolumn{1}{c}{0.8976 $\pm$ 0.005} &
  \multicolumn{1}{c}{0.7599 $\pm$ 0.008} \\
 \bottomrule
\end{tabular}%
}
\caption{Average validation/testing score comparison for each base method and corresponding homotopy approach across 5 separate seeds for the EVM experiments with MNIST dataset.}
\label{tab:table-exp-EVM-MNIST}
\end{table}

\begin{table}[ht!]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Method}} &
  \textbf{Validation F1} &
  \textbf{Validation Accuracy} &
  \textbf{Validation NMI} &
  \textbf{Testing F1} &
  \textbf{Testing Accuracy} &
  \textbf{Testing NMI} \\ \midrule
\multicolumn{1}{c}{\textbf{Random}} &
  \multicolumn{1}{c}{0.8556 $\pm$ 0.009} &
  \multicolumn{1}{c}{0.9659 $\pm$ 0.004} &
  \multicolumn{1}{c}{0.8254 $\pm$ 0.019} &
  \multicolumn{1}{c}{0.8191 $\pm$ 0.058} &
  \multicolumn{1}{c}{0.9596 $\pm$ 0.028} &
  \multicolumn{1}{c}{0.7927 $\pm$ 0.011} \\
\multicolumn{1}{c}{\textbf{PSHHO+Random}} &
  \multicolumn{1}{c}{0.8654 $\pm$ 0.004} &
  \multicolumn{1}{c}{0.9673 $\pm$ 0.001} &
  \multicolumn{1}{c}{0.8309 $\pm$ 0.009} &
  \multicolumn{1}{c}{\textbf{0.8248 $\pm$ 0.015}} &
  \multicolumn{1}{c}{0.9610 $\pm$ 0.002} &
  \multicolumn{1}{c}{0.7981 $\pm$ 0.011} \\
\multicolumn{1}{c}{\textbf{TPE}} &
  \multicolumn{1}{c}{0.8400 $\pm$ 0.018} &
  \multicolumn{1}{c}{0.9618 $\pm$ 0.006} &
  \multicolumn{1}{c}{0.8060 $\pm$ 0.026} &
  \multicolumn{1}{c}{0.7992 $\pm$ 0.026} &
  \multicolumn{1}{c}{0.9554 $\pm$ 0.005} &
  \multicolumn{1}{c}{0.7729 $\pm$ 0.024} \\
\multicolumn{1}{c}{\textbf{PSHHO+TPE}} &
  \multicolumn{1}{c}{0.8563 $\pm$ 0.016} &
  \multicolumn{1}{c}{0.9632 $\pm$ 0.007} &
  \multicolumn{1}{c}{0.8140 $\pm$ 0.030} &
  \multicolumn{1}{c}{0.8175 $\pm$ 0.014} &
  \multicolumn{1}{c}{0.9571 $\pm$ 0.005} &
  \multicolumn{1}{c}{0.7844 $\pm$ 0.023} \\
\multicolumn{1}{c}{\textbf{Bayes}} &
  \multicolumn{1}{c}{0.8426 $\pm$ 0.007} &
  \multicolumn{1}{c}{0.9617 $\pm$ 0.002} &
  \multicolumn{1}{c}{0.8049 $\pm$ 0.010} &
  \multicolumn{1}{c}{0.7919 $\pm$ 0.013} &
  \multicolumn{1}{c}{0.9542 $\pm$ 0.003} &
  \multicolumn{1}{c}{0.7657 $\pm$ 0.014} \\
\multicolumn{1}{c}{\textbf{PSHHO+Bayes}} &
  \multicolumn{1}{c}{0.8622 $\pm$ 0.008} &
  \multicolumn{1}{c}{0.9671 $\pm$ 0.003} &
  \multicolumn{1}{c}{0.8288 $\pm$ 0.016} &
  \multicolumn{1}{c}{0.8161 $\pm$ 0.015} &
  \multicolumn{1}{c}{0.9589 $\pm$ 0.003} &
  \multicolumn{1}{c}{0.78855 $\pm$ 0.015} \\
\multicolumn{1}{c}{\textbf{SMAC}} &
  \multicolumn{1}{c}{0.8510 $\pm$ 0.004} &
  \multicolumn{1}{c}{0.9657 $\pm$ 0.003} &
  \multicolumn{1}{c}{0.8241 $\pm$ 0.014} &
  \multicolumn{1}{c}{0.8218 $\pm$ 0.016} &
  \multicolumn{1}{c}{0.9602 $\pm$ 0.003} &
  \multicolumn{1}{c}{0.7951 $\pm$ 0.003} \\
\multicolumn{1}{c}{\textbf{PSHHO+SMAC}} &
  \multicolumn{1}{c}{\textbf{0.8698 $\pm$ 0.005}} &
  \multicolumn{1}{c}{\textbf{0.9699 $\pm$ 0.001}} &
  \multicolumn{1}{c}{\textbf{0.8433 $\pm$ 0.007}} &
  \multicolumn{1}{c}{0.8231 $\pm$ 0.010} &
  \multicolumn{1}{c}{\textbf{0.9613 $\pm$ 0.002}} &
  \multicolumn{1}{c}{\textbf{0.8001 $\pm$ 0.009}} \\
 \bottomrule
\end{tabular}%
}
\caption{Average validation/testing scores comparison for each base method and corresponding homotopy approach  across 5 separate seeds for the EVM experiment with LFW dataset.}
\label{tab:table-exp-EVM-LFW}
\end{table}
